Mobility and Transit Segregation in Urban Spaces

Segregation is a highly nuanced concept that researchers have worked to define and measure over the past several decades. Conventional approaches tend to estimate segregation based on residential patterns in a static manner. In this work, we analyse socioeconomic inequalities, assessing segregation in various dimensions of the urban experience. Moreover, we consider the pivotal role that transport plays in democratising access to opportunities. Using transport networks, amenity visitations, and census data, we develop a framework to approximate segregation, within the United States, for various dimensions of urban life. We find that neighbourhoods that are segregated in the residential domain, tend to exhibit similar levels of segregation in amenity visitation patterns and transit usage, albeit to a lesser extent. We identify inequalities embedded into transit service, which impose constraints on residents from segregated areas, limiting the neighbourhoods that they can access within an hour to areas that are similarly disadvantaged. By exploring socioeconomic segregation from a transit perspective, we underscore the importance of conceptualising segregation as a dynamic measure, while also highlighting how transport systems can contribute to a cycle of disadvantage.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
